Dimmer: Self-Adaptive Network-Wide Flooding with Reinforcement Learning

The last decade saw an emergence of Synchronous Transmissions (ST) as an effective communication paradigm in low-power wireless networks. Numerous ST protocols provide high reliability and energy efficiency in normal wireless conditions, for a large variety of traffic requirements. Recently, with the EWSN dependability competitions, the community pushed ST to harsher and highly-interfered environments, improving upon classical ST protocols through the use of custom rules, hand-tailored parameters, and additional retransmissions. The results are sophisticated protocols, that require prior expert knowledge and extensive testing, often tuned for a specific deployment and envisioned scenario. In this paper, we explore how ST protocols can benefit from self-adaptivity; a self-adaptive ST protocol selects itself its best parameters to (1) tackle external environment dynamics and (2) adapt to its topology over time. We introduce Dimmer as a self-adaptive ST protocol. Dimmer builds on LWB and uses Reinforcement Learning to tune its parameters and match the current properties of the wireless medium. By learning how to behave from an unlabeled dataset, Dimmer adapts to different interference types and patterns, and is able to tackle previously unseen interference. With Dimmer, we explore how to efficiently design AI-based systems for constrained devices, and outline the benefits and downfalls of AI-based low-power networking. We evaluate our protocol on two deployments of resource-constrained nodes achieving 95.8% reliability against strong, unknown WiFi interference. Our results outperform baselines such as non-adaptive ST protocols (27%) and PID controllers, and show a performance close to hand-crafted and more sophisticated solutions, such as Crystal (99%).

==> Figures/RL_model.tex <==
% \begin{tikzpicture}
%         % Environment Box
%         \draw[black,  thick,rounded corners] (2.8,0) rectangle (5.2,1) node[pos=.5] {Environment};
%         % Agent Box
%         \draw[black,  thick,rounded corners] (3,2) rectangle (5,3) node[pos=.5] {Agent};
%         % Action Arrow
%         \draw[very thick, ->] (5,2.5) -- (6.2,2.5) -- (6.2,0.5) node[midway, above, sloped] {\textit{action}} -- (5.2,0.5);
%         % Reward Arrow
%         \draw[very thick, ->] (2.8,0.6) -- (1.9,0.6) -- (1.9, 2.4) node[midway, below, sloped] {\textit{reward}} -- (3, 2.4);
%         % Observations Arrow
%         \draw[very thick, ->] (2.8,0.4) -- (1.7,0.4) -- (1.7, 2.6) node[midway, above, sloped] {\textit{observations}} -- (3,2.6);
% \end{tikzpicture}

==> Figures/deprecated/deep_Q_network.tex <==
\begin{tikzpicture}
        % Input
        \node[] (T0) {$T_0$};
        \node[right=of T0] (Tall) {\textbf{\dots}};
        \node[right=of Tall] (Tn) {$T_N$};
        \node[right= of Tn] (R0) {$R_0$};
        \node[right=of R0] (Rall) {\textbf{\dots}};
        \node[right=of Rall] (Rn) {$R_N$};
        \node[right=of Rn] (Ni) {$N_i$};
        % Deep layer
        \node[below=of R0] (deepmiddle) {\textbf{\dots}};
        \node[state, left= of deepmiddle] (deep1) {};
        \node[state, left= of deep1] (deep0) {};
        \node[state, right= of deepmiddle] (deepn1) {};
        \node[state, right=of deepn1] (deepn) {};
        % actions
        \node[state, below=of deepmiddle] (keepn) {};
        \node[state, left=of keepn] (decn) {};
        \node[state, right=of keepn] (incn) {};
        % actions text
        \node[below=of keepn] (keepntext) {$N$};
        \node[left=of keepntext] (decntext) {$N--$};
        \node[right=of keepntext] (incntext) {$N++$};
        % connect neurons
        % input to deep0
        \draw (T0.south) -- (deep0.north);
        \draw (Tn.south) -- (deep0.north);
        \draw (R0.south) -- (deep0.north);
        \draw (Rn.south) -- (deep0.north);
        \draw (Ni.south) -- (deep0.north);
        % input to deep1
        \draw (T0.south) -- (deep1.north);
        \draw (Tn.south) -- (deep1.north);
        \draw (R0.south) -- (deep1.north);
        \draw (Rn.south) -- (deep1.north);
        \draw (Ni.south) -- (deep1.north);
        % input to deepn1
        \draw (T0.south) -- (deepn1.north);
        \draw (Tn.south) -- (deepn1.north);
        \draw (R0.south) -- (deepn1.north);
        \draw (Rn.south) -- (deepn1.north);
        \draw (Ni.south) -- (deepn1.north);
        % input to deepn
        \draw (T0.south) -- (deepn.north);
        \draw (Tn.south) -- (deepn.north);
        \draw (R0.south) -- (deepn.north);
        \draw (Rn.south) -- (deepn.north);
        \draw (Ni.south) -- (deepn.north);
        
        
        % deep layer to action layer
        % deep to decn
        \draw (deep0.south) -- (decn.north);
        \draw (deep1.south) -- (decn.north);
        \draw (deepn1.south) -- (decn.north);
        \draw (deepn.south) -- (decn.north);
        % deep to keepn
        \draw (deep0.south) -- (keepn.north);
        \draw (deep1.south) -- (keepn.north);
        \draw (deepn1.south) -- (keepn.north);
        \draw (deepn.south) -- (keepn.north);
        % deep to incn
        \draw (deep0.south) -- (incn.north);
        \draw (deep1.south) -- (incn.north);
        \draw (deepn1.south) -- (incn.north);
        \draw (deepn.south) -- (incn.north);
        
        % action layer to action text
        \draw (decn.south) -- (decntext.north);
        \draw (keepn.south) -- (keepntext.north);
        \draw (incn.south) -- (incntext.north);
\end{tikzpicture}

==> Figures/deprecated/markov_goodbad.tex <==
\begin{scaletikzpicturetowidth}{0.1\textwidth}
\begin{tikzpicture}
        % states
        \node[fill=DMlightgreen, draw=DMdarkgreen, state] (g) {\textcolor{black}{\textbf{Good}}};
        \node[fill=DMlightred, draw=black, state, right= of g] (b) {\textcolor{black}{\textbf{\ Bad\ }}};
        
        % From states to states
        \draw[every loop]
            (b) edge[DMdarkgreen, bend right, auto=right] node {$0.2$} (g)
            (g) edge[DMdarkred, bend right, auto=right] node {$0.1$} (b)
            (b) edge[DMdarkred, loop right, very thick] node {$0.8$} (b)
            (g) edge[DMdarkgreen, loop left, very thick] node {$0.9$} (g);
        

\end{tikzpicture}
\end{scaletikzpicturetowidth}

==> Figures/deprecated/mdp_goodbad.tex <==
\begin{tikzpicture}[scale=0.7, every node/.style={transform shape}]
        % states
        \node[fill=DMlightgreen, draw=DMdarkgreen, state] (g) {\textcolor{black}{\textbf{Good RX}}};
        \node[fill=DMlightred, draw=black, state, below= of g] (b) {\textcolor{black}{\textbf{Bad/No RX}}};
        % actions
        \node[left= of g] (N_ten_g) {$P=10$ dBm};
        \node[right= of g] (N_one_g) {$P=0$ dBm};
        \node[left= of b] (N_ten_b) {$P=10$ dBm};
        \node[right= of b] (N_one_b) {$P=0$ dBm};
        
        % From states to actions
        \draw[thick, ->] (g) -- (N_ten_g);
        \draw[thick, ->] (g) -- (N_one_g);
        \draw[thick, ->] (b) -- (N_ten_b);
        \draw[thick, ->] (b) -- (N_one_b);
        
        % From actions to state
        % from good...
        % ...to good
        \draw[DMdarkblue, very thick, ->] (N_ten_g) to[out=160,in=110] (g);
        \draw[DMdarkorange, ->] (N_one_g) to[out=30,in=70] (g);
        % ...To bad
        \draw[DMdarkblue, ->] (N_ten_g) to[out=200,in=110] (b);
        \draw[DMdarkorange, very thick, ->] (N_one_g) to[out=340,in=70] (b);
        % from bad...
        % ...to good
        \draw[DMdarkblue, very thick, ->] (N_ten_b) to[out=160,in=250] (g);
        \draw[DMdarkorange, ->] (N_one_b) to[out=30,in=290] (g);
        % ...to bad
        \draw[DMdarkblue, ->] (N_ten_b) to[out=200,in=250] (b);
        \draw[DMdarkorange, very thick, ->] (N_one_b) to[out=340,in=290] (b);
        
\end{tikzpicture}

==> Figures/glossy_mdp.tex <==
% \begin{tikzpicture}[scale=0.8, every node/.style={transform shape}]
% %%% states
% % Good
%     \node[fill=white, draw=black, state] (g1)     {$2,Rx$};
%     \node[fill=white, draw=black, state, right=     of g1] (g2) {\textbf{$3,Rx$}};
%     \node[fill=white, draw=black, state, right=     of g2] (g3) {\textbf{$4,Rx$}};
% % Bad
%     \node[fill=white, draw=black, state,            below=of g1] (b1) {$2,\emptyset$};
%     \node[fill=white, draw=black, state,            below=of g2, right= of b1] (b2)             {\textbf{$3,\emptyset$}};
%     \node[fill=white, draw=black, state,            below=of g3, right= of b2] (b3)             {\textbf{$4,\emptyset$}};

       
% %%% From bar(Rx)|3
% % Maintain N 
%     \draw[->] (b2) edge[black, loop below,         very thick] (b2);
%     \draw[->] (b2) edge[black, bend left]     (g2);
% % Decrease N
%     \draw[->] (b2) edge[DMdarkorange, bend left,          in=180] (g1);
%     \draw[->] (b2) edge[DMdarkorange, bend left, very     thick] (b1);
% % Increase N
%     \draw[->] (b2) edge[DMdarkblue, bend right]           (b3);
%     \draw[->] (b2) edge[DMdarkblue, bend left, very       thick] (g3);
            
% \matrix [below] at (current bounding box.south) {
%   \node {
%     \scriptsize{\textbf{
%         \textcolor{DMdarkorange}{Decrease N}
%         \hspace{2em}
%         \textcolor{black}{Keep N}
%         \hspace{2em}
%         \textcolor{DMdarkblue}{Increase N}
%     }}
%   };\\ 
% };
% \end{tikzpicture}

% %\node [circle, label=right:Increase N] {}
%   %\node [circle, label=right:Keep N] {}

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	samples/sample-manuscript.tex \
	samples/sample-acmsmall.tex \
	samples/sample-acmlarge.tex \
	samples/sample-acmtog.tex \
	samples/sample-sigconf.tex \
	samples/sample-sigconf-authordraft.tex \
	samples/sample-sigconf-xelatex.tex \
	samples/sample-sigplan.tex \
	samples/sample-sigchi.tex \
	samples/sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

samples/%: %
	cp $^ samples

samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-sigconf-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done

samples/sample-manuscript.pdf \
samples/sample-acmsmall.pdf \
samples/sample-acmlarge.pdf \
samples/sample-acmtog.pdf: samples/samplebody-journals.tex

samples/sample-sigconf.pdf \
samples/sample-sigconf-authordraft.pdf \
samples/sample-sigconf-xelatex.pdf \
samples/sample-sigplan.pdf \
samples/sample-sigchi.pdf: samples/samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut

distclean: clean
	$(RM) $(PDF) samples/*-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf samples/sample-*.pdf *.cls *.bst

